SoundnessBench: Can Your AI Scientist Really Tell Good Research Ideas from Bad Ones?

Autonomous AI research agents aim to speed up scientific discovery by automating the research pipeline from hypothesis generation to peer review. However, existing benchmarks rarely test a fundamental bottleneck whether LLMs can judge the methodological viability of a research idea $\textbf{before}$ investing time and computational resources. Without a reliable ``first-gate'' filter, autonomous agents risk scaling flawed methodology rather than accelerating meaningful science. We introduce $\textbf{SoundnessBench}$, a curated benchmark of 1,099 real research proposals, with source verified extraction, reviewer-derived proxy labels, and proposal-only expert judgments on a subset of 327 proposals. Across 12 frontier LLMs, our evaluation reveals a pervasive $\textbf{optimism bias}$: standard prompting yields a $74.0\%$ mean false-positive rate. Aggressive prompting reduces false approvals but substantially increases false rejections. Additional analyses show that optimism persists under controls for public corpus contamination, and surface features, as well as in literature-grounded agent evaluation. These results suggest a limitation in judging scientific soundness, indicating that current LLMs are not yet reliable as standalone gatekeepers for scientific rigor.

==> assets/coordination-figure.tex <==
\begin{tikzpicture}[x=1cm,y=1cm,font=\sffamily\small,
  nodebox/.style={minimum width=3.7cm,minimum height=1cm,align=center},
  flow/.style={-{Stealth[length=5pt]},draw=APDark,line width=0.65pt}]
  \node[nodebox] (human) at (0,0) {\textbf{Human direction}\\[-1pt]\scriptsize Objectives and constraints};
  \node[nodebox] (agents) at (5.2,0) {\textbf{Agent coordination}\\[-1pt]\scriptsize Proposals and assignments};
  \node[nodebox] (eval) at (10.4,0) {\textbf{Evaluation}\\[-1pt]\scriptsize Evidence and feedback};
  % Explicit border anchors locate the arrow-start squares in either layout.
  \draw[flow] (human.east)--(agents.west);
  \apstart{human.east}
  \draw[flow] (agents.east)--(eval.west);
  \apstart{agents.east}
  % Name the two turns to place square junctions precisely in either layout.
  \coordinate (feedback-right) at ([yshift=-0.53cm]eval.south);
  \coordinate (feedback-left) at (agents.south |- feedback-right);
  \draw[flow] (eval.south)--(feedback-right)--(feedback-left)--(agents.south);
  \apstart{eval.south}
  \apbend{feedback-right}
  \apbend{feedback-left}
  \node[fill=white,inner sep=2pt,font=\ttfamily\tiny,text=APGray] at (7.8,-1.16) {UPDATE};
\end{tikzpicture}


==> assets/diagram-style.tex <==
% Load after TikZ. Mark an explicit right-angle turn with \apbend{coordinate};
% use \apbend[APAccent]{coordinate} to match a differently colored connector.
% Square connector markers are part of both paper and cover layouts.
% Mark an arrow's starting border with \apstart{node.east} or {node.south}.
\providecommand{\apbend}[2][APDark]{%
  \path[fill=#1,draw=none]
    ([xshift=-1.5pt,yshift=-1.5pt]#2) rectangle
    ([xshift=1.5pt,yshift=1.5pt]#2);
}
\providecommand{\apstart}[2][APDark]{\apbend[#1]{#2}}


==> design2.tex <==
% !TeX program = xelatex
% COVER LAYOUT PREVIEW (legacy filename: design2.tex)
% Overleaf: select this file as Main document; use XeLaTeX as Compiler.
% Separate ruled cover page; Introduction starts on page 2.
% Edit the manuscript and its options in main.tex. This wrapper forces only
% layout=cover, inheriting main.tex's theme, logo placement and all content.
% The default wordmark is below the abstract; add logo=top in main.tex to move
% it above the title. Main.tex contains the complete commented option guide.
% For a new paper, edit starter.tex and use layout=cover on its class line;
% these wrappers preview main.tex, not starter.tex.
\def\APResearchDesignOverride{2}
\input{main.tex}


==> sections/evaluation_results_old.tex <==
\section{Evaluation}


\subsection{Evaluation Setup}\label{sec:eval:setup}


\textbf{Models.}
We evaluate \textbf{12 frontier models} spanning small and large scales, non-reasoning and reasoning, and both closed- and open-source models. We includes GPT-4o, GPT-5.4-Mini, GPT-5.4, Claude-Opus-4.6, Claude-Sonnet-4.6, Gemini-2.5-Pro, Gemini-3-Flash, Gemini-3.1-Pro, Qwen-3.5-27B, Qwen-3.5-122B-A10B, LLaMA-3.3-70B, Kimi-Linear-48B-A3B.

\textbf{Inference Setup.} We run closed-source models through provider APIs and serve open-source models with vLLM on two NVIDIA H200 GPUs. We use \texttt{max\_tokens=8192} and \texttt{temperature=0.2}; other settings follow provider or framework defaults.

\textbf{Evaluation Protocol.}
We instruct LLMs to classify SoundnessBench proposals as high or low soundness, providing a detailed justification before the final label. We evaluate three settings: (1) \textit{Standard prompt}, which requests a structured assessment without an explicit conservative prior; (2) \textit{Aggressive prompt}, which instructs models to default to low soundness unless the idea and experimental design are clearly strong and well-justified; and (3) \textit{Literature-grounded scientific agent}, using ScholarEval~\citep{moussa2025scholareval}, a retrieval-augmented evaluator. Data-construction prompts and additional evaluation analyses are in Appx.~\ref{sec:supp:data-construction} and Appx.~\ref{sec:supp:evaluation}, respectively.



\textbf{Metrics.} We report confusion matrices, class-wise recall (Low R and High R), and Macro F1 (the unweighted average of per-class F1 scores). Low R measures rejection of low-soundness proposals, while High R measures identification of high-soundness proposals. Taking high soundness as the positive class, false positives (low$\rightarrow$high) reflect optimism, whereas false negatives (high$\rightarrow$low) reflect over-conservatism relative to the reference labels.



\subsection{Main Results under ICLR Proxy Labels}\label{sec:eval:main-results}\label{Sec: Main Results under ICLR Proxy Labels}

\begin{table}[!htbp]
\centering
% \renewcommand{\arraystretch}{1.0}
\caption{Summary evaluation metrics across 12 models under standard and aggressive 
prompting. Low R and High R denote recall on low- and 
high-soundness proposals. Macro F1 is the unweighted average of 
per-class F1 scores. Best Macro F1 per condition is \textbf{bolded}. 
$\dagger$ denotes reasoning model.}
\label{tab:main_results}
\resizebox{0.9\textwidth}{!}{%
\begin{tabular}{lcccccc}
\toprule
& \multicolumn{3}{c}{\textbf{Standard Prompt}} 
& \multicolumn{3}{c}{\textbf{Aggressive Prompt}} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-7}
\textbf{Model} 
& \textbf{Low R} $\uparrow$ & \textbf{High R} $\uparrow$ & \textbf{Macro F1} $\uparrow$
& \textbf{Low R} $\uparrow$ & \textbf{High R} $\uparrow$ & \textbf{Macro F1} $\uparrow$ \\
\midrule
\multicolumn{7}{l}{\textit{Open-source Models}} \\
LLaMA-3.3-70B          & 2.0  & 99.4 & 38.9 & 39.3 & 76.1 & 57.5 \\ % chktex 8
Kimi-Linear-48B-A3B    & 13.8 & 84.6 & 44.6 & 50.2 & 45.8 & 47.5 \\
Qwen3.5-27B$^\dagger$  & 23.6 & 92.5 & 55.1 & 83.8 & 32.4 & 52.6 \\ % chktex 8
Qwen3.5-122B-A10B$^\dagger$ & 26.6 & 90.6 & 56.3 & 95.6 & 16.8 & 44.7 \\ % chktex 8
\midrule
\multicolumn{7}{l}{\textit{Closed-source Models}} \\
GPT-4o$^\dagger$       & 5.5  & 98.9 & 42.3 & 87.1 & 25.0 & 48.5 \\
GPT-5.4-mini           & 50.7 & 76.6 & 63.8 & 100.0 & 0.2 & 29.7 \\
GPT-5.4$^\dagger$      & 64.6 & 74.6 & \textbf{69.7} & 100.0 & 0.0 & 29.5 \\
Gemini-2.5-Pro$^\dagger$         & 13.8 & 98.4 & 49.8 & 73.4 & 55.1 & 62.7 \\
Gemini-3-Flash         & 19.7 & 98.1 & 54.5 & 76.4 & 60.4 & 67.1 \\
Gemini-3.1-Pro$^\dagger$         & 26.0 & 96.1 & 58.4 & 89.1 & 35.9 & 57.0 \\
Claude-Sonnet-4.6$^\dagger$      & 37.2 & 94.8 & 65.3 & 94.4 & 18.8 & 46.0 \\
Claude-Opus-4.6$^\dagger$        & 28.2 & 97.2 & 60.5 & 72.2 & 66.4 & \textbf{68.6} \\
\midrule
\textbf{Mean}          & 26.0 & 91.8 & 54.9 & 80.1 & 36.1 & 49.3 \\
\bottomrule
\end{tabular}%
}
\end{table}

\begin{figure}[ht]
    \centering
    \includegraphics[width=0.95\linewidth,trim=0 0 0 0,clip]{figures/eval_confusion_all.pdf}
    \caption{Confusion matrices under the standard prompt across 12 evaluated models. Main message: many models are overoptimistic by default. The mean false-positive rate on low-soundness proposals is 74.0\% (9/12 models exceed 70\%). This pattern appears across model families in this evaluation setting.}
    \label{fig:eval-confusion-standard}
\end{figure}




We first evaluate all 1,099 proposals using the ICLR-derived proxy labels. Table~\ref{tab:main_results} reports class-wise recall and Macro F1 under standard and aggressive prompting.

% \paragraph{Standard prompting favors approval.} Across model families, models frequently classify proposals with low ICLR-derived soundness labels as high soundness. Mean low-soundness recall is 26.0\%, corresponding to a false-positive rate of 74.0\%, while mean high-soundness recall is 91.8\%. Nine of the 12 models classify more than 70\% of low-soundness proposals as high soundness. The strongest asymmetry appears in LLaMA-3.3-70B and GPT-4o, with false-positive rates of 98.0\% and 94.5\%, respectively. GPT-5.4 achieves the highest Macro F1 (69.7\%), with low- and high-soundness recall of 64.6\% and 74.6\%. These results indicate a broad tendency toward approval relative to the ICLR proxy labels.

\textbf{Across LLM families, we observe a pervasive optimism bias: models frequently rate proposals with low reviewer-derived soundness labels as sound.} As summarized in Tab.~\ref{tab:main_results} and visualized in Fig.~\ref{fig:eval-confusion-standard}, many proposals labeled as low soundness are predicted as high soundness. Specifically, under standard prompting, mean low-soundness recall is 26.0\% (equivalently, a 74.0\% false-positive rate), while mean high-soundness recall remains 91.8\%. At the model level, 9/12 models (including Gemini-3.1-Pro and Claude-Opus-4.6) label more than 70\% of low-soundness proposals as high soundness. The strongest optimism appears in LLaMA-3.3-70B and GPT-4o, which classify 98.0\% and 94.5\% of low-soundness proposals as high soundness. This pattern indicates that model judgments are often skewed toward approval even when proposal quality is limited. In practice, many default model configurations behave as permissive first-gate reviewers. Instead of consistently filtering weak proposals, they approve a broad set of candidates, which can lead to avoidable compute spend and weaker downstream experimentation.\ \tuyen{Representative false-positive and true-positive examples, together with concrete model responses, are provided in Appx.~\ref{sec:supp:qualitative-fp-tp}.} % chktex 8

\textbf{A few frontier LLMs reduce optimism bias, but at the cost of missing more high-soundness proposals.} For example, GPT-5.4 and GPT-5.4-mini are more conservative, but their high-soundness recall drops to 74.6\% and 76.6\%, respectively.\ \fh{This suggests a calibration trade-off in current frontier LLMs for proposal-stage soundness judgment: stricter filtering can suppress false approvals, but it also increases the risk of rejecting promising ideas.}

\textbf{Under Aggressive Prompting: Bias Shifts Toward Over-Conservatism.} The aggressive prompt reduces false approvals but increases false rejections. Mean false-positive rate falls from 74.0\% to 19.9\%, while high-soundness recall drops from 91.8\% to 36.1\%. Ten of the 12 models achieve false-positive rates below 30\%, but seven retain high-soundness recall below 40\%. At the extreme, GPT-5.4 and GPT-5.4-mini classify nearly all proposals as low soundness, with high-soundness recall of 0.0\% and 0.2\%, respectively. Thus, the tested stricter instructions improve rejection of low-soundness proposals at the expense of identifying high-soundness proposals.


% \tuyen{\textit{Adding a literature-grounded scientific agent does not resolve this optimism bias.} We additionally evaluate ScholarEval~\citep{moussa2025scholareval}, a retrieval-augmented scientific-idea evaluator, as a literature-grounded agentic scorer on matched SoundnessBench subsets. Unlike direct prompting, ScholarEval extracts proposed methods, retrieves and summarizes relevant prior work, assigns 0--10 method-level soundness scores, and averages them into an idea-level score. We follow the original ScholarEval source code and adapt it to evaluate SoundnessBench. On the coverage $\geq 0.8$ subset, even a strict score threshold of 8.0 still yields a 65.7\% false-positive rate on low-soundness proposals and F1 of 74.0\%, below direct standard prompting on the same subset (F1 84.4\%). Overall, adding literature grounding through a scientific agent is insufficient by itself for identifying the methodological flaws represented in SoundnessBench. Full protocol details and threshold sweeps are reported in Appx.~\ref{sec:supp:scholareval}.}

% \fh{\textit{The optimism bias is not simply a small-model artifact.} To isolate scale from model family and training recipe, we evaluate six models from the same Qwen3.5 family, ranging from 2B to 122B parameters, under both prompting conditions (Supplementary Fig.~\ref{fig:scale}). Under standard prompting, high-soundness recall improves with scale (71.8\% at 2B to 92.8\% at 35B), but low-soundness recall simultaneously decreases (31.0\% at 2B to 19.2\% at 35B). In other words, larger models become \textit{more} permissive toward weak proposals, not less. Under aggressive prompting, scale also provides no consistent recovery: all six models trend toward over-conservatism, with high-soundness recall ranging from 1.4\% (4B) to 32.4\% (27B) and no monotonic improvement with size.}



\subsection{\fh{Robustness Controls and Alternative Explanations}}\label{sec:eval:controls}

\fh{Because SoundnessBench is reconstructed from public ICLR papers and uses reviewer-derived soundness labels, we explicitly test whether the main optimism-bias pattern could be explained by label noise, extraction leakage, public-corpus contamination, paper recognition, shallow textual structure, or slice-level concentration. These controls do not make the benchmark contamination-free or convert reviewer scores into perfect ground truth; instead, they narrow the most plausible alternative explanations for the observed behavior.}

\begin{itemize}[leftmargin=*,itemsep=0in, topsep=0in, parsep=0in]
    % \item \tuyen{\textbf{Label and leakage audit.} A preliminary human verification audit checks whether extracted proposals leak results or outcome cues and whether reviewer-derived labels are defensible given only the extracted experiment plan and benchmark label shown to annotators. In the completed audited subset, 92.3\% of leakage checks match the expected ``No'' answer and 84.6\% of label-validity checks match the expected ``Yes'' answer (Appx.~\ref{sec:supp:human-audit}).}
    \item \fh{\textbf{Contamination and identifier controls.} As shown in Supplementary Tab.~\ref{tab:contamination_2026}, on an ICLR 2026-only split evaluated with cutoff-restricted models, low-soundness proposals are still predicted as high soundness at a similar rate to the full dataset (77.47\% vs. 73.88\%). Removing paper-identifying phrases changes the aggregate confusion matrix by roughly one percentage point (Appx.~\ref{sec:supp:contamination-control}, Sec.~\ref{sec:supp:identifier-removal}).}
    \item \fh{\textbf{Surface-feature and slice controls.} Simple no-training baselines based on proposal length, experiment count, and risk-factor count fail in the opposite direction from LLMs: they over-reject high-soundness proposals, whereas LLMs over-approve low-soundness proposals. The optimism bias also persists across years, primary areas, and writing-quality bands (Appx.~\ref{sec:supp:surface-baselines}, Sec.~\ref{sec:supp:slice-breakdowns}).}
    \item \fh{\textbf{Adversarial content control.} When severe hypothesis\textendash{}experiment mismatches are injected into 100 high-soundness proposals, GPT-5.4's approval rate drops from 77.0\% to 1.0\%, suggesting that models do attend to salient methodological content but remain insufficiently critical of subtler naturally occurring flaws (Appx.~\ref{sec:supp:adversarial-injection}).}
\end{itemize}

\tuyen{Overall, these analyses support a calibrated interpretation: SoundnessBench is an imperfect but audited proxy for recoverable proposal-stage soundness, and the observed optimism bias is unlikely to be explained solely by leakage, memorization, simple style features, or a narrow topic slice.}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.95\linewidth,trim=0 12 0 0,clip]{figures/eval_confusion_aggressive_all.pdf}
    \caption{Confusion matrices under the aggressive prompt across 12 evaluated models. Main message: optimism bias often shifts toward over-conservatism. The mean false-positive rate on low-soundness proposals drops to 19.9\% (10/12 models are below 30\%), but recall on high-soundness proposals also drops to 36.1\% (7/12 models are below 40\%). This illustrates strong prompt sensitivity in proposal-stage soundness judgment for the evaluated models.}
    \label{fig:eval-confusion-aggressive}
\end{figure}



\subsection{Under Aggressive Prompting: Bias Shifts Toward Over-Conservatism}\label{sec:eval:aggressive}\label{Sec: Under Aggressive Prompting: Optimism Bias Is Not Fixed, It Is Inverted}

\fh{\textit{The tested stricter prompt does not jointly improve both classes; it mainly shifts errors from false positives to false negatives.}} We observe widespread optimism bias in Sec.~\ref{sec:eval:main-results}. Motivated by this, we test how judgments change when the decision threshold is made deliberately stricter while keeping the same models and task: default to \textit{low soundness} unless the idea and experimental design are clearly strong and well-justified. Additional analyses for this setting are presented in Appx.~\ref{sec:supp:scale-bias} and Sec.~\ref{sec:supp:instruction-tuning-bias}. As shown in Tab.~\ref{tab:main_results} and Fig.~\ref{fig:eval-confusion-aggressive}, models generally become more conservative: low-soundness rejection improves, but high-soundness identification drops. The trade-off is quantitatively large. Mean low-soundness false positives drop from 74.0\% (standard prompt) to 19.9\% (aggressive prompt), and 10/12 models are below 30\%; meanwhile, mean high-soundness recall drops from 91.8\% to 36.1\%, with 7/12 models below 40\%. At the extreme, GPT-5.4 and GPT-5.4-Mini move to near-always-low behavior under aggressive prompting: low-soundness false positives are 0\% for both, while high-soundness recall falls to 0.0\% and 0.2\%, respectively. Other models show the same pattern in milder form; for example, Qwen3.5-122B-A10B and Claude-Sonnet-4.6 strongly reject low-soundness ideas (95.6\% and 94.4\% rejection), but correctly identify only 16.8\% and 18.8\% of high-soundness proposals. Consistent with this, mean Macro F1 decreases from 54.9 to 49.3. % chktex 8

\fh{\textit{Taken together, these results point to a prompt-sensitive capability limitation in proposal-stage judgment.}} Prompt sensitivity varies substantially across models. Remarkably, GPT-5.4 has the best Macro F1 under standard prompting (69.7\%) but drops sharply under aggressive prompting (29.5\%), whereas Claude-Opus-4.6 changes much less (60.5\% vs.\ 68.6\%). This cross-model variation, together with the robustness analyses (Sec.~\ref{sec:eval:controls}; Appx.~\ref{sec:supp:instruction-tuning-bias} and Sec.~\ref{sec:supp:scale-bias}), suggests that the optimism bias is prompt-sensitive, persists across tested model scales, and is not removed by instruction tuning within the examined family.



\begin{tcolorbox}[colback=green!5,colframe=teal!60!black,boxrule=0.8pt]
\fh{\textit{\textbf{Key Takeaway 1.}} Frontier LLMs show a broad optimism bias: models frequently rate low-soundness proposals as sound under standard prompting.} 

\medskip
\fh{\textit{\textbf{Key Takeaway 2.}} The tested stricter prompt does not jointly improve discrimination on both classes; it mainly shifts errors from false positives to false negatives.}

\medskip
\fh{\textit{\textbf{Key Takeaway 3.}} Taken together, results point to a prompt-sensitive capability limitation in proposal-stage soundness judgment: current LLMs are not yet reliable as standalone gatekeepers for scientific rigor.}
\end{tcolorbox}

==> sections/intro-old.tex <==
\section{Introduction}

Autonomous AI research agents are becoming increasingly capable. Recent systems can generate ideas, write code, run experiments, and draft papers with limited human intervention~\citep{lu2024aiscientist, yamada2025aiscientistv2, schmidgall2025agentlab, karpathy2026autoresearch}. This progress is promising, but it also exposes a core bottleneck: before implementation starts, an agent must decide whether a proposed idea and experimental plan are scientifically sound. In human research, this first-gate judgment often determines whether weeks of work and substantial compute are invested or avoided.

\paragraph{Research Gap.} Existing evaluations rarely test this decision point directly. Current benchmarks~\citep{chan2024mle,starace2025paperbench,wu2025innovatorbench,lupidi2026airs} for research agents mainly emphasize execution, such as reproducing papers or delivering runnable research artifacts, rather than testing whether an agent can judge if a proposed idea and experimental design are worth pursuing in the first place. This leaves an important upstream question unanswered: can an LLM reliably reject weak research proposals before execution?

This question is especially important because scientific triage depends on stable decision behavior. Prior work on sycophancy and prompt fragility suggests that model judgments can shift with framing~\citep{sharma2024sycophancy, syntacticfragility, causalt5k}. If this also happens in scientific triage, autonomous agents may scale poor decisions rather than accelerate robust discovery.

\textbf{In this paper}, we introduce SoundnessBench, a benchmark for pre-execution scientific judgment. We reconstruct it from real ICLR submissions with reviewer metadata and expert assessments from ML researchers. We derive high/low soundness labels from high-agreement reviews, extract near-verbatim hypothesis--experiment proposals without revealing experimental outcomes, and verify extraction faithfulness with retrieval-backed atomic-claim auditing. The resulting dataset contains 1,099 hypothesis--experiment proposals spanning 39 ICLR primary areas.

We evaluate 12 frontier LLMs on SoundnessBench. Under standard prompting, models show a clear optimism tendency: they often classify low-soundness proposals as high soundness, with a mean false-positive rate of 74.0\%, while high-soundness recall remains high (91.8\%). We then run a second evaluation with an aggressive prompt that explicitly encourages skepticism. This reduces low-soundness false positives to 19.9\%, but high-soundness recall also drops to 36.1\%, indicating over-correction.

These findings suggest that current frontier LLMs are not yet reliable first-gate scientific critics on this benchmark. Their judgments are often inaccurate on low-soundness cases and sensitive to prompt framing. In practice, this instability can allow weak proposals through under one prompt and filter out strong proposals under another. To further assess robustness, we provide additional analyses on model scale and base-versus-instruction-tuned behavior in Supplementary Sec.~\ref{sec:supp:scale-bias} and Sec.~\ref{sec:supp:instruction-tuning-bias}.

\begin{table*}[t]
\centering
\renewcommand{\arraystretch}{1.3}
\caption{Comparison of SoundnessBench with related benchmarks for evaluating 
LLMs in research contexts. \textbf{Stage} refers to when in the research pipeline 
the benchmark operates. \textbf{Input} is what the LLM receives. \textbf{Ground 
Truth} is the source of labels. \textbf{Soundness Focus} means the benchmark 
directly tests methodological rigor. \textbf{Pre-Exe. Judgment} means the 
benchmark tests the model before any experimental results are known.}
\label{tab:benchmark_comparison}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lccccccc}
\toprule
\textbf{Benchmark} & \textbf{Stage} & \textbf{Task} & \textbf{Input} 
& \textbf{Ground Truth} & \textbf{Soundness} & \textbf{Pre-Exe.} 
& \textbf{Verified} \\
 & & & & \textbf{Source} & \textbf{Focus} & \textbf{Judgment} 
& \textbf{Extraction} \\
\midrule
MLE-Bench         
& Exe.     & Engineering   & Full task spec      
& Kaggle outcome        & \rx & \rx & \rx \\

PaperBench      
& Exe.     & Replication   & Full paper + code   
& Human rubric          & \rx & \rx & \rx \\

InnovatorBench      
& Exe.     & Research loop & Task description    
& Outcome metric        & \rx & \rx & \rx \\

AIRS-Bench      
& Exe.     & Multi-task    & Full paper          
& Expert annotation     & \rx & \rx & \rx \\

ResearchGym
& Exe.     & Research loop & Task description    
& Outcome metric        & \rx & \rx & \rx \\

\midrule

Si et al. \small{(2025)}                      
& Ideation      & Idea ranking  & Idea text           
& Human study           & \rx & \gck & \rx \\

Hindsight               
& Post-hoc      & Impact pred.  & Full paper          
& Citation count        & \rx & \rx & \rx \\

Schopf \& Färber \small{(2026)}               
& Post-hoc      & Novelty judge & Abstract            
& Expert label          & \rx & \gck & \rx \\

Tong et al. \small{(2026)}                    
& Post-hoc      & Taste ranking & Full paper          
& Citation / venue      & \rx & \rx & \rx \\

\midrule

\textbf{SoundnessBench}                
& \textbf{Pre-exe.} & \textbf{Soundness judge} 
& \textbf{Proposal} & \textbf{Expert label}  
& \gck & \gck & \gck \\

\bottomrule
\end{tabular}%
}
\end{table*}

\paragraph{Our contributions are:}
\begin{itemize}
    \item We introduce SoundnessBench, a benchmark that isolates pre-execution scientific soundness assessment from real ML submissions. It provides a shared testbed for comparing methods and analyzing first-gate filtering behavior in autonomous research systems.
    \item We provide a reconstruction pipeline with explicit reliability controls: reviewer-agreement filtering, near-verbatim proposal extraction, and retrieval-backed atomic-claim verification for faithfulness.
    \item We present an empirical study across 12 frontier LLMs, showing a broad optimism tendency under standard prompting and a shift toward over-conservative behavior under aggressive prompting. We further provide supplementary analyses on scaling and instruction tuning (Supplementary Sec.~\ref{sec:supp:scale-bias} and Sec.~\ref{sec:supp:instruction-tuning-bias}), highlighting prompt sensitivity as an important challenge for compute-efficient autonomous research agents.
\end{itemize}

